Analytical Model of Memory-Bound Applications Compiled with High Level Synthesis

The increasing demand of dedicated accelerators to improve energy efficiency and performance has highlighted FPGAs as a promising option to deliver both. However, programming FPGAs in hardware description languages requires long time and effort to achieve optimal results, which discourages many programmers from adopting this technology. High Level Synthesis tools improve the accessibility to FPGAs, but the optimization process is still time expensive due to the large compilation time, between minutes and days, required to generate a single bitstream. Whereas placing and routing take most of this time, the RTL pipeline and memory organization are known in seconds. This early information about the organization of the upcoming bitstream is enough to provide an accurate and fast performance model. This paper presents a performance analytical model for HLS designs focused on memory bound applications. With a careful analysis of the generated memory architecture and DRAM organization, the model predicts the execution time with a maximum error of 9.2% for a set of representative applications. Compared with previous works, our predictions reduce on average at least $2\times$ the estimation error.

==> Tips_for_programmers.tex <==
*Increasing the number of buffers to be accessed to external memory decrease the memory throughput due to DRAM have to changes row or pages that are the most expensive operations, for this reason, when the access are continuous, structs are convenient.

*Increase the LSU_widht increases the burst length but the kernel frequency is decrease.

*The take advantage of the DRAM architecture, all the continuous access are tried to be coalesced to reduce precharge and activation commands using the burst mode, even if the detected access worst access pattern as write.-ack

*To increase the memory access performance in continuous access, the memory architectures are advancing to multiply the number of banks, hiding latency and kernel computation

*The FIFO structures to pass data between different clock domains,and the avalon interface allows to pass asyncronous data between kernel and the memory controller. (AValon FIFO).

*the restrict word in kernels allows to compiler simplify arbitration hardware.
%The data form kernel arrvies at different times, and shoul be wait in a queue, in a FIFO structucture, allowing asynchronous, due to the finite size of a FIFO, the data flow should be controlled to prevent the overflow
%the different domain clocks can hides the

*With the new characteristics of load/store in 19.3 with instructions like __prefetching_load this model would be more accurate, avoiding computational instructions, and saturating the memory, when is possible.

==> old_motivation.tex <==
% Dario, this file is not in use

\section{Motivation}

Due to synthesis on FPGAs is time expensive, performance analysis models for FPGAs using HLS tools \ruben{esto no es solo de hls, vendria bien independientemente del framework de trabjao}are designed to guide and tune codes with less compilation time. This model have to involve to main components: computation and memory behavior.

Memory is one of the main bottlenecks on FPGA for HPC applications\ruben{cita?}. Memory bound applications covers a lot of applications, this is why it is of great importance to know their performance\ruben{???}. Proposed models do not cover the interconnection layer between external memory controller and the kernel. This interconnection can change the data transfer rate introducing control structures that modify the number of kernel access cycles to memory, and with this the estimated value.

For example, in HPCA model \ruben{cita a los autores y referencia}, they have a fixed memory transaction width, based on hardware specifications and have dependencies with the SIMD/unroll vectorization. Furthermore, this model does not take into account the memory frequency limiting the model to the memory used on evaluated system.
To show the differences between the predicted model and the measured time the figure Fig.\ref{fig:motivation_time} shows a vector add NDRange microbenchmark with a coalesced memory access.

%Sngelica
%For example, in HPCA model, validated on a Stratix V FPGA , they have a fixed memory transaction width, based on hardware specifications and have dependencies with the SIMD/unroll vectorization. Furthermore, this model do not take in account the memory frequency limiting the model to the memory used on the base system.
%In contrast, the memory cycles measurements on this paper, validated on a Stratix10 GX FPGA, shows dependencies on the dynamic memory width, that is \angelica{defined} on global memory interconnect prior to synthesis; even though the memory width changes with the SIMD/unroll, it is a discontinuous mathematical relation.  To show this, we implement a vector add NDRange microbenchmark with a coalesced memory access, the Fig\ref{fig:motivation_time} shows the calculated bandwidth using the HPCA model and measured.



 \begin{figure}[!htbp]
\centering
\includegraphics[width=0.71\columnwidth]{figure/Motivation_HPCA_time.pdf}
\caption{Estimated and measured time on Vector-Add application with variation of SIMD and number of inputs vectors. }
\label{fig:motivation_time}
\end{figure}

The error introduced by the model changes the direction that programmers takes to optimize algorithms, guiding them to reduce the SIMD factor with consequences on degradation of memory bandwidth and part of exploration space to optimized the programs is ignored.

To improve the cycles estimation on memory bound applications, this paper explores the architecture dependencies on global memory interconnect, taking as parameters the defined prior to synthesis to guide the programmers to optimizations knowing inside the global memory interconnection.







% On Hotspot, a Rodinia benchmark optimized for FPGA architectures \cite{Zohouri2016}, the authors use a technique to reduce the number of global memory access, this optimization requires stride global memory access and small chunks of data with small computation in every run. The intermediate compilation report in fig\ref{fig:Hotspot} shows that the global memory interconnect is composed by two memory load units and one store of type: burst-coalesced no aligned. 
 
%  \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.7\columnwidth]{Hotspot.png}
% \caption{System viewer from memory report for Hotspot}
% \label{fig:Hotspot}
% \end{figure}

% The profiled results of this shows a bandwidth of 8.9 of 14.9GB\/s  maximum possible  for a DDR4 1866, due to the stride memory access. With the model proposed in this paper, we can capture the memory bandwidth of the application in 8.5GB\/s. This results is with a vectorization of 8 given by default for a Stratix V FPGA.

% We increase the vectorization 8$\times$ that can be resource supported in a new generation of FPGA Stratix10GX, This increases the memory width of the LSU units. With this change the measured bandwidth is 10.9 GB\/s and our model obtains 10.1GB\/s. In table \ref{tab:bw_hotspot} we compare the results.

% \ctable[
% caption = {Hotspot bandwidth measured and estimated by model in this work.},
% label=tab:bw_hotspot,
% pos=tbp,
% doinside = \small
% ]{lcc}{}
% { \FL
% \NN
%     Vector Size &   BW measured [GB/s] & BW estimated   \ML
%     8           &   8.9             & 8.5    \NN
%     64          &   10.9            & 10.1
% \ML
% }



%AHora la motivación queda pendiente.


%Memory  are specified by the memory device vendor, and the type of memory controller . The 
%the type of LSU are generated by the compiler after intermediate compilation. The heuristic optimization cost function on Intel compiler has defined a three main objectives, first, a hardware memory oriented implementation with stall-free load\/stores units; second, a hardware with the maximum frequency and the last is optimize the resource utilization.
